Fast and Space-Efficient Parallel Algorithms for Influence Maximization

Influence Maximization (IM) is a crucial problem in data science. The goal is to find a fixed-size set of highly-influential seed vertices on a network to maximize the influence spread along the edges. While IM is NP-hard on commonly-used diffusion models, a greedy algorithm can achieve $(1-1/e)$-approximation, repeatedly selecting the vertex with the highest marginal gain in influence as the seed. Due to theoretical guarantees, rich literature focuses on improving the performance of the greedy algorithm. To estimate the marginal gain, existing work either runs Monte Carlo (MC) simulations of influence spread or pre-stores hundreds of sketches (usually per-vertex information). However, these approaches can be inefficient in time (MC simulation) or space (storing sketches), preventing the ideas from scaling to today's large-scale graphs. This paper significantly improves the scalability of IM using two key techniques. The first is a sketch-compression technique for the independent cascading model on undirected graphs. It allows combining the simulation and sketching approaches to achieve a time-space tradeoff. The second technique includes new data structures for parallel seed selection. Using our new approaches, we implemented PaC-IM: Parallel and Compressed IM. We compare PaC-IM with state-of-the-art parallel IM systems on a 96-core machine with 1.5TB memory. PaC-IM can process large-scale graphs with up to 900M vertices and 74B edges in about 2 hours. On average across all tested graphs, our uncompressed version is 5--18$\times$ faster and about 1.4$\times$ more space-efficient than existing parallel IM systems. Using compression further saves 3.8$\times$ space with only 70% overhead in time on average.

==> algo.tex <==
% \section{Algorithms}\label{sec:alg}

% \input{tab_algorithms.tex}

% brief summary to talk about we will present the details about the ``sketch'' and ``update priority'' parts in Algorithm 1.
Our algorithm (as well as most sketch-based algorithms) has two phases: sketch construction (named sketching) and seed selection (named selecting). 
The challenges of running IM on large-scale graphs come from two aspects, one is memory usage, the other one is running time. 
We optimized memory usage by proposing a compact sketching algorithm, which provides a method to trade-off between running time and memory usage. 
Besides, we optimized running time by parallelizing the CELF seeds selection process by introducing two parallel data structures to maintain the vertices sorted by their marginal influences.  They could increase parallelism without introducing many extra re-evaluations compared to CELF.
% The details of compact sketching and parallel selecting are in Sec \ref{sec:compact_sketching} and Sec \ref{sec:selecting}.


\input{cc.tex}


\input{tree.tex}

==> cover_page.tex <==
% \begin{titlepage}
    \thispagestyle{empty}
    \twocolumn[
    \begin{center}
     %\centering
     \Huge Response to Reviewer's Comments \\~
     \end{center}
    ]

    \balance 
    We thank the reviewers for their constructive suggestions and comments.  In this letter, we summarize how we address the required and optional changes in the meta-review, as well as other revisions to address the individual comments from reviewers. We hope that these changes have addressed the reviewers' concerns. In this letter, we keep pointers to \revision{Sections}, \revision{Figures}, \revision{Tables}, and \revision{Algorithms} in the \textbf{revised paper}, which is attached at the end of this cover letter. We have also highlighted the modified components in a different \revision{color} for easy identification.

    We also made other minor changes and shrank some figures in the paper to fit the page limitation. For some additional experimental results and proofs that cannot fit in the 12-page paper, we provide them in the full version of the paper~\cite{influencemaximizationfullpaper2023}.


\section{Enhance the Technical Analysis}
    \begin{tcolorbox}
        \textbf{1.} How to optimally select the center vertices for sketch compression? Currently, they are selected uniformly at random, but will some centrality-based selection (e.g., betweenness centrality, PageRank centrality, etc.) be more effective? [Reviewer 1 D1(a)]
    \end{tcolorbox}
    We thank Reviewer 1 for this interesting question. The purpose of center selection is to use the information stored per center to efficiently recover the connected component (CC) information of any vertex in the graph.
    In our algorithm, we choose to select centers uniformly at random in all vertices. This is to \emph{ensure the theoretical guarantee in \cref{thm:sketch}}:
    a vertex can recover the CC information by either encountering a center in $1/\alpha$ steps of BFS or traversing its entire CC, whose cost is bounded by $O(\min(1/\alpha, T_r))$, where $\alpha$ is the sample rate and $T_r$ is the CC size of the vertex on the $r$-th sketch.

    We agree that using centrality-based centers is an interesting heuristic. However, we did not find a similar theoretical guarantee for such centers. One other complication here is that the centrality properties of sketches (sampled graphs) may differ from those of the original graph, which is affected by the propagation rates of each edge. In other words, the top $k$ vertices in a centrality measurement on the original graph may not still be the top $k$ on the sketches. 

    In summary, in this paper, we \emph{use the randomly selected centers for the theoretical guarantee, and leave more heuristics for center selection as future work}. \revision{We added a short discussion in \cref{sec:compact_sketching} after \cref{thm:sketch}.}

    \hide{, i.e., a vertex can recover the CC information by either encountering a center in $1/\alpha$ steps of BFS or traversing its entire CC, whose cost is bounded by $O(\min(1/\alpha, T_r))$, where $\alpha$ is the sample rate and $T_r$ is the CC size of the vertex on the $r$th sketch (see \revision{\cref{thm:sketch}} for more details).}
    \hide{
    However, the performance of centrality-based center selection relies on the exact centrality measure and the topological properties of the graphs, for which we can not find any theoretical guarantee of recovering CC information. }
    \hide{
    However, we can not find a similar theoretical guarantee for centrality-based center selections.
    % Therefore, in the theory aspect,  centrality-based selection won't be more effective.
    % On the other hand
    Besides, the centrality properties of sketches (sampled graphs) may be different from those of the original graph because different edge propagation rates are assigned to different edges according to the propagation model. In other words, the top $k$ vertices in a centrality measurement on the original graph may not still be the top $k$ on the sketches. We think how to apply centrality measurement as heuristics may be an interesting future work. \revision{We added a short discussion in \cref{sec:compact_sketching} after \cref{thm:sketch}.}}



    \begin{tcolorbox}
        \textbf{2.} It could be discussed why only forward sketches are considered, and if there are any limitations in considering reverse-reachable sketches. [Reviewer 1 D1(b)]
    \end{tcolorbox}
    % There is no limitation in applying \ptree{} and \WinTree to reverse-reachable sketches.
    We thank Reviewer 1 for bringing up this question. The difference between reverse-reachable and forward-reachable algorithms is how they construct sketches and compute the marginal influence $\truegain{v}$ according to their sketches.
    \emph{Our compression technique is designed for forward-reachable sketches, so we focus on forward-reachable algorithms in this paper.} We note that our parallel CELF algorithm \emph{potentially applies to reverse-reachable algorithms, which we briefly discuss below.}

    Both reverse-reachable and forward-reachable algorithms are based on the greedy algorithm introduced in the paper. 
    We can either update the $\truegain{v}$ actively or lazily in both categories. Active updating means that the algorithm decreases the marginal influence of related vertices immediately after selecting a seed to ensure $\truegain$ is always up to date. Lazy updating (CELF) means only re-evaluating $\Delta(v)$ if the stale marginal value $\lazygain{v}$ is the largest among the remaining vertices.  Our \ptree{} and \wintree are parallel optimizations for lazily updating (CELF). 
    Most existing reverse-reachable sketch algorithms~\cite{minutoli2019fast, cohen2014sketch} use active updating, which may involve certain optimizations specific to each reverse-reachable algorithm. 
    To use our new data structures, we can replace their seed selection scheme with our new parallel CELF as a general seed selection idea.

    We thank the reviewer for pointing out this interesting direction, and agree that it is interesting to apply \ptree{s} and \wintree{s} to reverse-reachable algorithms. We note that to achieve the best results for the reverse-reachable algorithms, we may also need to improve the parallelism/space usage of the sketch construction step of the reverse-reachable algorithms, which is beyond the scope of this paper. \revision{We leave them as future work and we added a short discussion in \cref{sec:related} and \cref{sec:conclusion}.}


    \begin{tcolorbox}
        \textbf{3.} Do the compression and parallelization techniques work with other propagation models besides IC? [Reviewer 1 D1(c)]
    \end{tcolorbox}
    We thank Reviewer 1 for the insightful question. We also believe it is important to carefully understand the generality of our algorithms. In particular, as we briefly mentioned in \cref{sec:intro}, the parallel data structures for seed selection can be applied to other propagation models with the submodular property, which is true for most commonly used models, such as IC and linear threshold~\cite{kempe2003maximizing}. Since CELF itself is a general technique for optimization problems with submodularity, we believe our new data structures can potentially provide good parallelism for other optimization problems with submodular objectives, too.

    % The compression technique only works for the IC model on undirected graphs.
    The compression technique requires the sampled graphs (sketches) to be undirected so that memoization can be used, i.e., a vertex activates all vertices in the same connected component (CC) when the edges are sampled with the propagation probabilities. 
    The essential requirement is that edge $u \to v$ and edge $v \to u$ in the original graph always have the same probability of being sampled. This is true for the IC model on undirected graphs, but is not always true for other models, such as Linear Threshold. 
    This property has been observed and used in previous work~\cite{chen2009efficient,gokturk2020boosting}. 
    Therefore, \oursystem{} has the same limitation as these previous approaches, i.e., it applies to the IC model and requires the graph to be undirected. 

    \revision{To address the comment, we discuss the generalization and limitations of our techniques in \cref{sec:conclusion}.}

    \hide{1) the connected component (CC) size of a vertex is its influence if no vertex inside the CC is selected as seed 2) the vertices in the same CC have the same influence score.
    The essential requirement for undirect sketches is that edge $u \to v$ and edge $v \to u$ in the original graph always have the same probability of being sampled.
    Among all the propagation models as far as we know, the IC model on undirected graphs is the only one that meets this requirement, so our compression model is only applicable to the IC model on undirected graphs. \revision{We discuss the limitations of our techniques in \cref{sec:conclusion}.} }

    % because only under such a setting do the vertices inside the same connected component have the same influence spread, which is the connected component size.
    \begin{tcolorbox}
        \textbf{4.} It would be better to provide a formal discussion on the correctness and cost bound of the win-tree solution. [Reviewer 3 D1]
    \end{tcolorbox}
    We thank Reviewer 3 for this useful comment. Although the correctness analysis is more straightforward than \ptree{s}, we agree that it is useful to provide the analysis for \wintree{s} for completeness. Due to the page limit,
\revision{we provided a formal discussion on the correctness of \wintree{} in the full version of this paper but gave some intuitions in \cref{sec:WinTree}.} %The correctness is proofed in two steps: we first proof the tree $T$ maintains a valid \wintree after calling \textsc{NextSeed}, then proof $\truegain{T.root}=\max_{v\in V} {\truegain{v}}$.

    Unlike \ptree{}, we can not provide a strong cost bound for the number of evaluations in \wintree{} since the parallel threads are highly asynchronous. 
    They do not explore the \wintree{} layer by layer but in a non-deterministic order. Therefore, the worst-case cost can be high in theory. However, the ``worst-case'' is very unlikely in practice, and we observed good performance for \wintree{} in experiments. \revision{We briefly discuss this in \cref{sec:conclusion}.}

\section{Improve the experimental analysis}\label{sec:exp-cover}
    \begin{tcolorbox}
        \textbf{1.} Clarification for the term `relative influence'. Why the `relative influence' of competing methods do not reach $100\%$? Are they approximate? However, why does the proposed method always reach $100\%$? [Reviewer 1 D2(a)]
    \end{tcolorbox}
    We thank Reviewer 1 for this clarification question. The ``relative influence'' is the influence spread normalized to the maximum influence spread selected by \ours{} ($R=256$),  \infuser{} ($R=256$), and \ripples{} ($\epsilon=0.5$). The value of maximum influence is shown in \cref{tab:graph_info}. Because the IM problem is NP-hard, we cannot know the actual optimal influence of each test. Therefore, we compare the influence value of each system to the best among them to indicate the solution quality of each algorithm. 
    \revision{We move the definition of relative influence to the caption of \cref{tab:baselines} to make it easier to find.} 

    
    
    As mentioned, since the IM algorithm is NP-hard, all existing algorithms are approximate because they cannot find the actual ``optimal'' influence. 
    \oursystem{} and all tested baselines are based on the classic greedy algorithm, which is $(1-1/e)$-approximate. However, the approximation ratio assumes that the marginal gain can be computed exactly. 
    In practice, the marginal gain is computed by Monte Carlo simulations, with the tradeoff between the round of simulations and accuracy. 
    \oursystem{} and baseline algorithms have parameters to control the round of simulations (number of sketches), $R$ for \oursystem{} and \infuser{} and $\epsilon$ for \ripples. Larger $R$ or smaller $\epsilon$ means better accuracy but costs more time and space. For fairness in the performance comparison (in time and space), we always set the parameters for \oursystem{} ($R$), \infuser{} ($R$) and \ripples{} ($\epsilon$) in the way that \oursystem{} has a higher influence spread than baseline algorithms (mentioned in \revision{\cref{sec:exp}, Paragraph \textbf{\textit{Tested Algorithms}}}). 
    This demonstrates a better performance of \oursystem{} even when it also yields better solution qualities.
    The relative influence is the influence spread normalized to the highest score on each graph. Because \oursystem{} is always higher than baseline algorithms, the relative influence for \oursystem{} is always $100\%$, and that for baseline algorithms is always less than $100\%$. 
    By adjusting the parameters, the baseline algorithms can achieve a higher influence in most cases but make their running times significantly slower than the reported ones in the paper. 
    

    % For the sketch-based algorithm, there is a parameter to control the trade-off between the influence spread and the number of sketches. The higher the influence spread wanted, the more sketches are needed. For forward-sketch algorithms, such as \ours{} and \infuser, that is $R$; for backward-sketch algorithms, such as \ripples{}, that is $\epsilon$. If the algorithm is implemented correctly, \ours{} and \infuser{} should have a similar influence spread on the same graph, because we choose the same $R$. However, due to some implementation issues, such as data races, \infuser{} does not get the influence spread as well as \ours{}.

    \begin{tcolorbox}
        \textbf{2.} How are the edge probabilities assigned, and how do different edge probability distribution impacts the proposed methods? [Reviewer 1 D2(b) and Reviewer 3 D2]
    \end{tcolorbox}
    We thank Reviewers 1 and 3 for asking this. We assigned the edge probabilities according to related works for scale-free graphs. As this is the first paper to test IM on sparse graphs, we set the probability empirically to make the tests non-trivial (explained in more detail below). Below we use $p_{uv}$ to denote the edge probability of edge $(u,v)$, or directly use $p$ with clear context. 
    
    For the edge probability on social networks, previous work~\cite{chen2009efficient, kim2013scalable, cohen2014sketch, gokturk2020boosting} mostly chose a fixed value of $p$ from $\{0.01, 0.02, 0.1\}$. We simply choose $p=0.02$ for social and web graphs. For the sparse graphs (road and $k$-NN graphs), note that they are sparser and the degrees of vertices are usually no more than 5. 
    In this case, using $p=0.02$ may cause most vertices to be unable to impact any other vertices. To make the tests non-trivial, we choose $p=0.2$ for road and $k$-NN graphs.

    % We also tested different edge probability distributions and saw their impact. We
    To study how different edge probability distributions will affect \oursystem{} and baselines algorithms, we also tested two more edge probability distributions. The first is based on uniform distribution, which is also commonly seen in previous papers~\cite{gokturk2020boosting, minutoli2019fast}. We denote $U(x,y)$ as a uniform distribution between real numbers $x$ and $y$. We set the propagation probability for each edge as $U(0,0.1)$ for social and web graphs, and $U(0.1,0.3)$ for road and $k$-NN graphs. The second one is to take $p_{uv}=\frac{2}{d_u+d_v}$, where $d_u$ and $d_v$ are degrees of vertex $u$ and $v$. It is similar to the Weighted IC (WIC) model on the directed graph, where $p_{uv} = \frac{1}{d_{in}(v)}$, and $d_{in}(v)$ is the in-degree of vertex $v$. In these two distributions, instead of a fixed $p$, the edge probability can differ for different edges. 


    Overall, both \ours{1} and \ours{0.1} have the fastest running times than all baselines in time on \emph{all but the two smallest graphs} for each tested edge probability assignment. In those exceptions, \ours{1} has a running time very close to \infuser{}, much shorter than \ripples{}. 
    \ours{0.1} has lower space usage on \emph{all} tested edge probability assignments and graphs. 
    The relative performance is fairly consistent on these three edge probability distributions.

    \revision{We provide detailed experiment results and discussions in the appendix of the full version paper, and briefly summarize the conclusions in \cref{sec:exp}, Paragraph \textbf{\textit{Setup}}.}  
    \revision{We also provide them at the end of the cover page for easy access.}
    Since the relative performance for different edge probability distributions is similar, we simply use the version with a fixed probability $p$ for all edges to demonstrate the performance in the main body of the paper.

    \hide{In general, we found the relative performance among the tested algorithms, on all tested propagation probability distributions, are mostly the same as what we show in the main paper. \oursystem{} has better performance than the baselines in both time and space on all tested edge probability assignments. The performance comparison between \oursystem and baseline algorithms are similar on Consistent ($p=0.02$ for scale-free graphs and $p=0.2$ for sparse graphs) and Uniform assignments. \ripples performs differently on WIC because it dynamically samples sketches while \oursystem and \infuser sample fixed $R$ sketches.
    \revision{We add how we set the edge propagation rate and how different edge distributions influence the performances of \oursystem and baselines in \cref{sec:exp}.}
    }

    \begin{tcolorbox}
        \textbf{3.} In Section 5.2, it is mentioned that the proposed techniques scale well up to 8-16 cores on many graphs, but the performance may deteriorate with more cores. It would be valuable to provide some insights or possible explanations for this observation. Exploring the reasons behind this behavior would add depth to the discussion [Reviewer 3 D3]
        % \xiangyun{I think the reviewer made a mistake here. Our method does not have scalability issues. Only ripples and infuser do have.}
    \end{tcolorbox}
    %\letong{please have a look, don't know how to answer.}
    If the `proposed techniques' refer to \oursystem{}, we apologize for the confusion and thank Reviewer 3 for pointing this out. Our algorithm \emph{did not} exhibit scalability issues in our experiments using up to 192 threads (shown in \cref{fig:scale}). We guess there may be two parts in \cref{sec:scalability} that caused the misunderstanding. We point them out here and hope we can explain them more clearly. 

    1. (Original paper)  ``\textit{For \oursystem{}, both sketch and selection
    time decreases with more cores and achieves almost linear speedup.
    Unfortunately, such a scalability trend is not always true for \infuser{} and \ripples{}.
    They scale to 8--16 cores on many graphs,
    but the performance may get worse with more cores.}''.

    Here, the scalability issues occur in \infuser{} and \ripples{}. 
    On many graphs, their performance drops with more than 16 cores, but \oursystem{} still benefits with more than 16 cores. This can also be seen in \cref{fig:scale}.


    2. (Original paper) ``\textit{Even for \ours{1} where the selection time is a small fraction of the total running time when $P=1$,
    the sequential selecting time is still much longer than the total running time when $P>16$.}''

    In this case, we meant that \emph{if} we did not parallelize the seed selection part, then it would become a performance bottleneck when $P>16$. This statement is to illustrate the necessity of proposing new parallel data structures for the seed selection step. In fact, due to our techniques in \cref{sec:selecting}, the seed selection step scaled well and did not become the performance bottleneck of the entire computation.

    \revision{For both of the sentences above, we rephrased them in \revision{\cref{sec:scalability}}.}

    If the `proposed techniques' refer to the two baseline algorithms \infuser{} and \ripples{}, we briefly discussed their scalability issues \revision{at the end of \cref{sec:scalability}}, and provide a more detailed discussion here.  As mentioned in \cref{sec:scalability}, \infuser{} and \ripples{} scale better on sketch construction than seed selection because they use well-parallelized algorithms to construct sketches. For seed selection, they only parallelize the work of one evaluation across different sketches, and all evaluations are performed one by one. 
    For both \infuser{} and \ripples{}, the actual computation for one evaluation is reasonably quick (e.g., for \infuser{}, it only needs to read the stored CC size on each sketch and add them up). 
    In this case, the overhead of scheduling the parallel threads can be more expensive than the computation (and even dominate the cost), which increases with the number of threads. 
    Therefore, when $P$ is large, an evaluation may be more expensive when running in parallel than sequential. 
    On scale-free networks where a large number of evaluations are required, the overhead accumulates, which results in the poor performance of \infuser{} on SLDT, LJ, and SD in \cref{fig:scale}. 
    %For each re-evaluation, these approaches need to fork and join $P$ threads for each seed evaluation, so the parallel overhead increases with more cores, which may even be much larger than the actual work of evaluation.  
    %Therefore, the scalability issue for seed selection is especially obvious on graphs that have a large number of evaluations (such as social and web graphs). 


    \hide{for \ours{1}, even though the selection time takes only a small fraction of the total sequential running time when $P=1$, the selection time under $P=1$ is still much longer than the total time under $P>16$.  }
    
    

    \begin{tcolorbox}
        \textbf{4.} Provide experiment results to show the number of re-evaluations in each round in CELF to justify the need for improving the parallelism [Reviewer 3 D4]
    \end{tcolorbox}
    We thank Reviewer 3 for this advice.
    \revision{We experimentally study the distribution of $|F_i|$ among $i$ from 1 to $k$ on graphs. We show the results on three representative graphs in \cref{fig:celf_evaluations} and provide some discussions in \cref{sec:selecting}.}
    Among all the tested graphs, the evaluation distributions across the rounds show three patterns:
    \begin{itemize}
        \item Social and web graphs (e.g., LJ) usually need a large number of evaluations close to $n$ at the beginning. The subsequent evaluations are in a smaller range.
        \item The road graphs (e.g., GER) usually have no more than 5 evaluations in each round. 
        \item For $k$-NN graphs (e.g., CH5), the number of evaluations varies in a large range (about $10$–$10^4$ for CH5) across rounds.
    \end{itemize}

    We show an example for each of the three patterns in \cref{fig:celf_evaluations}.
    According to the experiment results, CELF re-evaluates more than $10^3$, even more than $10^5$ (for social and web graphs) vertices for many graphs in certain rounds. This demonstrates the necessity of parallelizing CELF.
    \hide{
    \revision{We discuss the three distribution patterns of re-evaluations at the beginning of \cref{sec:selecting}.}}

    \begin{tcolorbox}
        \textbf{5.} Explain why the comparison with state-of-the-art only focuses on \infuser{} and \ripples{}. [Reviewer 4 W2]
    \end{tcolorbox}
    \infuser{}, \ripples{} and \NoSingles{} are \emph{the best multi-core parallel implementations} that we know of. 
    They cover two main sketch-based algorithm categories: \infuser{}, a forward-reachable sketch algorithm; and \ripples{} and \NoSingles{},  reverse-reachable sketch algorithms. 
    As mentioned in the paper, \ripples{} is always superior to \NoSingles{} in both time and space metrics. Therefore, we only report \ripples{} as a representative of the parallel reverse-reachable sketch algorithm.

    We have also tested some sequential algorithms, such as PMC~\cite{ohsaka2014fast} and IMM~\cite{tang2015influence}, but their running times are not competitive to the parallel solutions. 
    In particular, they are slower than \oursystem{} on all graphs, and slower than \infuser{} on most of the graphs. \revision{We add a discussion about the choice of baseline algorithms in \cref{sec:exp}, Paragraph \textbf{\textit{Tested Algorithms}}. }



\section{Discuss the potential limitations of the proposed solution}

    \begin{tcolorbox}
        \textbf{1.} Can you add a discussion of the potential limitations of the proposed solution, e.g., can the parallel priority queue solution be easily extended for another computational model that may not guarantee shared memory access? [Reviewer 3 general comment]
    \end{tcolorbox}
    We thank Reviewer 3 for this useful comment. 
    In a nutshell, as we mentioned in the paper, our sketch compression algorithm is limited to undirected graphs and the IC model. 
    The parallel data structures for seed selection are more general: they only require the objective function to be submodular, which is true for most commonly used models, such as IC and Linear Threshold~\cite{kempe2003maximizing}.

    For the specific question in this comment, we also discuss it here. While the data structures themselves require some non-trivial adaptions to be applied in other computational models (e.g., distributed memory), some high-level ideas, such as prefix-doubling, are applicable. For example, with an existing distributed search tree that supports batch operations, we can use it to replace \ptree{s} in our prefix-doubling idea. This will lead to a CELF algorithm in the distributed memory setting.

    For \wintree{s}, it seems possible to extend it to distributed settings by distributing disjoint sub-trees to different computational nodes. When running \textsc{NextSeed}, we can work on different subtrees in parallel, and find the maximum among them. This may cost higher overhead in the distributed setting than shared memory, but it can still gain parallelism. To design an efficient version of \wintree{} for IM in the distributed setting may need more non-trivial optimizations, which is beyond the scope of this paper.

    \revision{In the revised version, we summarize the limitations of our proposed techniques, their potential generalizations, and interesting future directions in \cref{sec:conclusion}.} 


    \hide{We proposed \ptree{} and \wintree{} to parallelize CELF and we will discuss them respectively.
    For the \ptree{} method, we can break it down into three basic operations: popping candidates, re-evaluating candidates and batch insertion. Re-evaluation can be directly parallelized as each re-evaluation is independent of the other. Popping candidates is essentially to find the $i$-th element or split at the $i$-th element in a Binary Search Tree (BST), which is done by one thread. If you can find an implementation of BST that supports batch insertion in the desired computational model, you can extend our \ptree method by replacing the \ptree with that BST implementation.



    For the \wintree{} method, you can also extend it to another computational model that does not support shared memory access. If you look at a certain layer of a \wintree, you will find several disjoint sub-trees that are still valid \wintree{s}. You can distribute sub-trees to different computational nodes. When querying the \textsc{NextSeed}, different threads can find the vertex with maximum marginal gain on different sub-trees in parallel, and find the maximum among them. This method may cost more computation than the original \wintree{} method mentioned in the paper, but it can still gain parallelism. }

% \newpage
\input{appendix}


% \end{titlepage}
% \clearpage
% \pagenumbering{arabic}
% \newpage
\clearpage
\setcounter{section}{0}


==> figures/fig_CELF_eval_all.tex <==
\begin{figure}[th]
  \centering
  \includegraphics[width=\columnwidth]{figures/CELF_eval_all.pdf}
  \caption{\small \textbf{The number of evaluations done by CELF in each round.} Each point $(x,y)$ represents CELF does $y$ number of re-evaluations in the $x$-th round.
  \label{fig:celf_evaluations}}
\end{figure} 

==> figures/fig_compact.tex <==
\begin{figure*}[th]
  \centering
  \includegraphics[width=\textwidth]{figures/compact_figures.pdf}
  \caption{\small \textbf{compact IM breakdown (in seconds) and memory (in GB).}  $y$-axis is the running time in seconds and memory usage in GB.
  \label{fig:compact_total}}
\end{figure*} 

==> figures/fig_evaluates.tex <==
\begin{figure}[th]
  \centering
  \includegraphics[width=0.9\columnwidth]{figures/evaluates.pdf}
  \caption{\small \textbf{Compare the number of re-evaluates between \ptree and \WinTree{}.} Each point represents a graph, whose $x$-index is the total number of re-evaluates that CELF does and $y$-index is that of \ptree (circle)/ \WinTree (triangle).
  \label{fig:evaluates}}
\end{figure} 

==> figures/fig_tree.tex <==
\begin{figure}[th]
  \centering
  \includegraphics[width=0.9\columnwidth]{figures/tree_time.pdf}
  \caption{\small \textbf{Compare the selection running time between \ptree and \WinTree{}.} Each point represents a graph running under a certain compression rate, whose $x$-index is the selection time of \WinTree and $y$-index is the selection time of \ptree. $c$ represents the compression rate. The red line represents $y=x$, above each means \ptree takes more time in selection than \WinTree.
  \label{fig:tree-time}}
\end{figure} 

==> figures/fig_trees.tex <==
\begin{figure}[th]
  \centering
  \includegraphics[width=\columnwidth]{figures/trees_violin.pdf}
  \caption{\small \textbf{Compare \ptree and \WinTree{} in the number of re-evaluations and selection time.} Figure (a) shows the comparison in 
 the number of re-evaluations, where each point represents a test case whose $x$-index is \#re-evaluations needed in CELF, and $y$-index is that needed in \ptree (blue circle) or \WinTree (orange triangle). The red line is $y=x$. A point above it means a test case that parallel priority queues evaluate more vertices than CELF. 
 % The figure (b) shows the comparison in selection time, where each point represents a test case whose $x$-index is the selection time of \WinTree and $y$-index is that of \ptree. The red line represents $y=x$. A point above it means a test case where \ptree takes more time than \WinTree in seed selection.
 Figure (b) shows the distribution of \ptree selection time/\WinTree selection time under different $\alpha$. The three little bars mean the maximum, mean and the minimum of the data. The red horizontal line is $y=1$. 
 \yihan{May be useful to change (a) also to similar dot-figure as (b)}
\label{fig:trees}}
\end{figure} 

==> imp.tex <==
\section{Implementation} \label{sec:imp}

Infuser: More specifically, in our algorithm, for an edge $(u,v)$ and sketch id $r$, we defined $\hash\_edge(u,v,r)$ as \[\hash\_edge(u,v,r)\gets \hash(r) \oplus \hash(min(u,v)\ll 32 | max(u,v))\]
An edge $(u,v)$ is in the $r$\_th sampled graph if $\hash\_edge(u,v,r) < p(u,v)$

BST is from the PAM library

Union-find is from the ConnectIt library

Get-center allocates a local queue


